GPULZ: Optimizing LZSS Lossless Compression for Multi-byte Data on Modern GPUs

Today's graphics processing unit (GPU) applications produce vast volumes of data, which are challenging to store and transfer efficiently. Thus, data compression is becoming a critical technique to mitigate the storage burden and communication cost. LZSS is the core algorithm in many widely used compressors, such as Deflate. However, existing GPU-based LZSS compressors suffer from low throughput due to the sequential nature of the LZSS algorithm. Moreover, many GPU applications produce multi-byte data (e.g., int16/int32 index, floating-point numbers), while the current LZSS compression only takes single-byte data as input. To this end, in this work, we propose GPULZ, a highly efficient LZSS compression on modern GPUs for multi-byte data. The contribution of our work is fourfold: First, we perform an in-depth analysis of existing LZ compressors for GPUs and investigate their main issues. Then, we propose two main algorithm-level optimizations. Specifically, we (1) change prefix sum from one pass to two passes and fuse multiple kernels to reduce data movement between shared memory and global memory, and (2) optimize existing pattern-matching approach for multi-byte symbols to reduce computation complexity and explore longer repeated patterns. Third, we perform architectural performance optimizations, such as maximizing shared memory utilization by adapting data partitions to different GPU architectures. Finally, we evaluate GPULZ on six datasets of various types with NVIDIA A100 and A4000 GPUs. Results show that GPULZ achieves up to 272.1X speedup on A4000 and up to 1.4X higher compression ratio compared to state-of-the-art solutions.

==> sections/abstract.tex <==
%% moved

==> sections/background.tex <==
%% moved

==> sections/conclusion.tex <==
%% moved

==> sections/design.tex <==
%% moved

==> sections/encoding-kernel.tex <==
After we get all the matching results from the matching kernel, we need to use that to encode data. In the design of \culzss, this process is implemented on the CPU. Although CPU could be asynchronous while GPU is finding a match for the next chunk of data. The data movement time from CPU and GPU could cause a huge overhead for this process. Besides, the sequential operations make this step more time-consuming. Since our match result could only find a match inside a data block, we use GPU to parallel this process to gain maximum performance. The design of our encoding kernel is shown in \FIG \ref{fig:encode-kernel}.
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/encode_kernel.png}
    \caption{The structure of encoding kernel.}
    \label{fig:encode-kernel}
    %   \vspace{-6mm}
\end{figure}

\subsection{Data Partition}

The data partition we apply in the encoding kernel is different from the matching kernel because the granularity of data has changed. We use one thread to process the whole data block in the matching kernel. And then we store the encoded data in the global memory. Because of the characteristic of the data block, the match will not exceed the data block. Therefore, we can parallelize this process by mapping them to different threads simultaneously since they are independent of each other. Unlike the sequential version of LZSS, the former result of a data block does not affect the encoding of the next data block. This will cause a drop in the compression ratio. But as we analyzed before, it won't cause too many drawbacks to it. The maximum size of extra bytes for a data block of 4096 bytes is 2 bytes.

Due to the uncertainty in the compressibility of different data blocks in encoding, it takes longer to finish one data block than another; therefore, it causes the divergence between threads, leading to a drop in performance. What is worse, the measure of the divergence degree could be highly data-dependent and non-deterministic. 
% Thus, Tghuysrather, it is statisticalnot measurable. 
Thus, we make the match distribution statistically even by assigning a sufficiently large data block size, which corresponds to less divergence.
% We want to make the size of data block as big as possible to make the distribution of matches in different data blocks more similar. 
% So the divergence in different threads become smaller. 
% In the meanwhile, we do not want this data block too small neither. 
On the other hand
Because the smaller the data block is, the more extra bytes caused by data blocks will be. After we test a few options, we find that 4096 is a relatively good choice. So for now we apply 4096 as the data block size.
\subsection{Workflow Design}

The original design in the \culzss{} does not implement the pipeline arrangement to fully utilized the concurrency of GPU and CPU to increase the performance. The encoding thread in the CPU waits till the GPU matching kernel finishes to start encoding. And the matching kernel does not start to find a match till the former chunk of data is encoded. The structure is shown in \FIG \ref{fig:encode-diff} (a). This design makes the encoding process badly paralleled. Even after implementing the CPU and GPU concurrency, the D2H (Device to Host) time still causes unnecessary data movement time. Therefore, instead of focusing on implementing an optimized CPU version of the encoding kernel, we propose and develop a new GPU encoding kernel.

After replacing the CPU encoding function with the GPU encoding kernel, the workflow is demonstrated in \FIG \ref{fig:encode-diff} (b). The matching result is stored in GPU global memory, and the encoding kernel directly uses it without memory movement. Besides saving time for data movement, according to our evaluation, the GPU encoding kernel is also faster than CPU encoding.
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/encode_diff.png}
    \caption{The structure of CPU encoding kernel.}
    \label{fig:encode-diff}
    %   \vspace{-6mm}
\end{figure}

However, this is not the optimized solution. Due to the granularity of the encoding kernel being very coarse, it does not fully utilize the resources in GPU. Especially when we partition the data into chunks. Therefore, we only execute the encoding kernel once to encode the whole input stream after all the matching result is ready. It is shown in \FIG \ref{fig:encode-diff} (c). This design makes encoding kernel leverage as many GPU resources as it can. And it has the same execution time as the encoding kernel in (b) ideally. The speed up depends on the number of chunks. The more chunks there are, the more time is saved. Because the matching kernel fully utilizes the GPU resources in every iteration, this design does not cause waste of GPU SM resources.

According to our evaluation result, the total time of the GPU encoding kernel is smaller than the single iteration of the CPU encode kernel. And with the optimization for avoiding data movement. The total speedup achieves as high as 5.48x. And the detail of our encoding kernel design is illustrated in Alg.\ref{alg:encoding-kernel}.

\begin{algorithm}[b]
    \caption{Encoding Kernel.}
    \label{alg:encoding-kernel}
    \footnotesize
    \SetAlgoLined
    \KwIn{Matching result}
    \KwOut{Encoded data, Header}
    \textit{\_\_shared\_\_}  \textit{tmp\_buffer[\,]}\\
    ${int}$  ${coding\_position}$\\
    ${int}$  ${flags\_count}$\\
    ${unsigned\,char}$  ${flags}$\\
    \While{${n < data\_block\_size}$}
    {
        \While{${flags\_count < 8}$}
        {
            $index=(coding\_position+n)*2$\\
            \uIf{${matching\_result[index]==1}$}
            {
                $flags++$\\
                $flags<<1$\\
                $save\,to\,tmp\_buffer$
            }
            \Else
            {
                $flags<<1$\\
                $save\,to\,tmp\_buffer$
            }
        }
        $write\_out(flags)$\\
        $write\_out(tmp\_buffer)$\\
        $reset\,flags\,and\,flags\_count$\\
    }
    $save\,size\,to\,header$\\
    $save\,tmp\_buffer\,to\,encoded\_data$
\end{algorithm}

% \begin{lstlisting}[language=python, otherkeywords={__shared__, unsigned, char, output, matchInfo, struct, variable}]
% input: Matching result
% output: Encoded data, Header
% variable list:
% __shared__  tmp_buffer[]
% int coding_position, flags_count
% unsigned char flags

% while n < data_block_size:
%     while flags_count < 8
%         index <- (coding_position + n) * 2
%         if matching_result[index] == 1:
%             flags++
%             flags << 1
%             save to tmp_buffer
%         else:
%             flags << 1
%             save to tmp_buffer
%     write_out(flags)
%     write_out(tmp_buffer)
%     reset flags and count

% save size to header$
% save tmp_buffer to encoded_data
% \end{lstlisting}


==> sections/experiment.tex <==
%% moved

==> sections/introduction.tex <==
%% moved

==> sections/matching-kernel.tex <==
Due to the original design in \culzss{} is for general purpose compression. It wastes a lot of GPU resources when applying to scientific data lossy compression. We propose a new matching kernel more suitable for quantization code derived from {\cusz} for scientific data. We achieve a higher compression ratio by adding intervals to the matching kernel and finely tuning the window size. With full utilization of shared memory in GPU, we further significantly improve the performance.

\subsection{Data Partition}
The data partition is a significant part of the matching kernel. Because the chunk size directly affects the balance between compression ratio and performance. And it's also related to the thread block size allocation. Our data partition strategy is illustrated as \FIG \ref{fig:data-partition}.
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/data_partition.png}
    \caption{Input stream is divided and padded to fit GPU architecture.}
    \label{fig:data-partition}
    %   \vspace{-6mm}
\end{figure}
Our matching kernel aims to find the longest match for the bytes in the input stream and store them for later use. However, the size of the input stream is generally much larger than the number of allowed threads in modern GPUs. Therefore, we first partition the input sequence into smaller chunks to fit the GPU capacity. And we add padding to the last chunk if it's not full. The padding is meaningless data. We process one chunk at each iteration.
Then we divide the chunk into smaller data blocks and map them to thread blocks. Each data block corresponds to a thread block. Because the shared memory is shared in a thread block, and the size of shared memory is limited. Therefore, we want to allocate the proper size of the data block to make the matching kernel leverage the shared memory without overloading the shared memory. For example, we take 4096 bytes as the data block size. It is worth mentioning that the data block size in the matching kernel is the same as the data block size in the encoding kernel, which we will discuss in the next section.

\subsection{Interval and Window Size}
After partitioning the data into the right size we can process for GPU kernel; we need to find a match for every byte in the data buffer. However, suppose we continue to use the one-to-one mapping strategy for scientific data. In that case, it will cause a huge waste of GPU resources due to the match length in quantization code being generally very large. As a result, a lot of match results will be skipped.
Therefore, we proposed a new design with intervals inserted into the mapping strategy; we only find a match for bytes that has a certain distance from each other. For all the other bytes we do not find a match for, we treat them as if there is no match found for those bytes. It can significantly reduce the operations needed for the matching kernel. Because of the long match length character of scientific data, the trade-off on compression ratio will be relatively small. The interval is a customized variable, we take 1, 2, 4, 8, and 16 as the options for an interval. If the interval is 1 it would be the same as the original version of \culzss. If we take interval as more than 1, the threads number we need decreases from $numthreads$ to $numthreads/interval$, leading to a performance increase. We take an interval of 2 as an example; the matching kernel structure after adding an interval is demonstrated in \FIG \ref{fig:matching-kernel}.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{images/matching_kernel.png}
    \caption{The structure of original match kernel and interval version match kernel.}
    \label{fig:matching-kernel}
    %   \vspace{-6mm}
\end{figure}

On the other hand, if we increase the interval, the total number of matches we find will be less. It leads to a decrease in compression ratio. For example, we assume that the interval is 4. As illustrated in \FIG \ref{fig:interval}, byte 19 is encoded as a pointer if we use the original design of \culzss{} (i,e,. interval distance 1). And byte 20 is included in the match of byte 19. However, due to the interval, it is now encoded as a literal. This drawback is weaker as the match length grows; if the match length is generally long enough, then we can waste these bytes for a $1/4$ of total threads number.
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/interval.png}
    \caption{The structure of original match kernel and interval version match kernel.}
    \label{fig:interval}
    %   \vspace{-6mm}
\end{figure}
In the original design, the window size is a fixed number 128, which is enough for general purpose LZSS compression. However, according to our experience, the quantization code of scientific data generally has repeated patterns with a length more than 128. We count the length of matches for quantization code from 2 datasets, CESM and NYX. As a comparison, we also have statistics of normal data. The normal datasets are enwik8, and enwik9 from \textit{Large Text Compression Benchmark} \cite{enwik}. The result is shown in \FIG \ref{fig:statistics}.
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/fig4_rev1.pdf}
    \caption{The structure of original match kernel and interval version match kernel.}
    \label{fig:statistics}
    %   \vspace{-6mm}
\end{figure}
The match length in a scientific dataset is generally longer than normal data. And a big part of matches has a length of more than 256. This makes it possible to increase the compression ratio by extending the window size from 128 to 256. We use a window size of 256 instead of a longer window because the match length and offset is stored both using one byte. However, the window size increase means the number of operations in the matching kernel increases too. Due to the interval we add, the number of threads is decreased. Assume we use an interval of 2, then the number of threads is halved. After extending the window size from 128 to 256, we still have the same number of threads as the original design, which means the computation time is the same ideally, with the compression ratio increased. The drawback of wasting bytes by adding intervals is also weaker.

It is also worth mentioning that adding an interval will not introduce other wasted bytes other than the bytes skipped by the interval. As illustrated in \FIG \ref{fig:interval-matching}, Match Y in our design has the same ending position as Match X in the original design at least. Because no matter where in the sliding window Match X is, after the window slides across the skipped byte B0, a match is 1 byte shorter than Match X is in the new sliding window, which is Match Y. This guarantees that there are no other wasted bytes. In some specific situations, Match Y is even longer than Match X.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/interval_matching.png}
    \caption{The structure of original match kernel and interval version match kernel.}
    \label{fig:interval-matching}
    %   \vspace{-6mm}
\end{figure}

\subsection{Matching Strategy}

Matching is a very time-consuming process in the sequential version of LZSS compressor. It takes the time complexity of O(n\^{}2) in the worst case. And it's not stable, which is not suitable for the GPU kernel. Therefore, we apply the match-finding strategy in \culzss{} to minimize the divergence between different threads.
The algorithm is summarized as:
\begin{enumerate}[label=\arabic*), noitemsep, topsep=2pt, leftmargin=1.3em]
    \item We keep two pointers, one points to the start of the window, and the other points to the coding position.
    \item Keep adding two pointers till the byte two pointers point to is not the same.
    \item Record the current match length and offset, if it's longer than the recorded pointer before, then record this one instead, or skip it.
    \item Make the second pointer point to the coding position again and add 1 to the first pointer. Repeat step 2).
\end{enumerate}
This algorithm does not guarantee the optimized result, but it will output a relatively good result and is very stable since the time complexity is always O(n). And according to our knowledge, it will not output the best result only in very few situations.

Another thing to mention here, different from traditional LZSS, the max coded length is not allowed to exceed the offset. This is because we want to minimize the divergence between threads.

\subsection{Utilization of Shared Memory}
\culzss{} uses a loop array in the GPU shared memory to store all the look-ahead buffer bytes for the matching kernel to find a match. However, with every iteration in the matching kernel, the shared memory needs to be updated with new buffer data. This causes a huge overhead with many context switches in the kernel. After fully investigating the structure of the whole design, we use the data block size of 4096 bytes, which will make the desired data size for a thread block 4 KB. And the allowed shared memory for a single SM is capable of putting all of these bytes. Therefore, we re-design the kernel to move all the corresponding memory to shared memory once at the start of the kernel. And unlike \culzss's design, which writes the result of the match to global memory in every iteration. We also applied a shared memory temporary buffer to hold all the results for the matching kernel. According to our experiments, this leads to a speedup of 2x.

Due to the shared memory size, all the matches, which we find at the end of a data block, do not exceed the data block. That means when we try to find the longest match for a specific byte close to the end of the data block, the match length will be limited to the length of the remaining bytes of that data block, which is because the look-ahead buffer is running out and we can't find a match outside of the look-ahead buffer. It leads to a decrease in compression ratio, but it will only add at most 2 extra bytes to the output buffer since the next data block can at least find the original match length cut by the data block.

The detail of our matching kernel is illustrated in Algorithm \ref{alg:matching-kernel}.
\begin{algorithm}[b]
    \caption{Matching Kernel.}
    \label{alg:matching-kernel}
    \footnotesize
    \SetAlgoLined
    \KwIn{Input stream}
    \KwOut{Matching result}
    ${\_\_shared\_\_}$  ${input\_stream[\,data\,block\,size]}$\\
    ${\_\_shared\_\_}$  ${matching\_result[\,data\,block\,size*2]}$\\
    ${int}$  ${coding\_position}$\\
    ${int}$  ${window\_position}$\\
    ${matchInfo}$  ${match}$\\
    \ForEach{index in interval position}
    {
        load input stream to ${input\_stream}$ \\
    }
    ${threads\_synchronization()}$\\
    ${position\_initialization()}$\\
    \ForEach{index in interval position}
    {
        ${match=find\_match(coding\_position,\,window\_position)}$\\
        ${write\_out(matching\_result,\,match)}$ \\
        \ForEach{${n < interval\,size}$}
        {
            ${match.length=1}$\\
            ${match.offset=input\_stream[index+n]}$\\
            ${write\_out(matching\_result,\,match)}$ \\
        }
    }
    ${threads\_synchronization()}$\\
    \ForEach{index in interval position}
    {
        write ${matching\_result}$ back to global memory\\
    }
    %\vspace{-4mm}
\end{algorithm}
% \begin{lstlisting}[language=python, otherkeywords={__shared__, unsigned, char, output, MatchInfo, struct, variable}]
% input: input stream
% output: matching result
% variable list:
% __shared__ input_stream[data_block_size]
% __shared__ matching_result[data_block_size * 2]
% int coding_position, window_position
% struct MatchInfo { int length, offset } match

% for index in C:
%     load input stream to input_stream
% threads_synchronize()
% position_initialize()
% for index in C:
%     match <- find_match(coding_position, window_position)
%     write_out(matching_result, match)
%     while n < interval_size:
%         match.length <- 1
%         match.offset <- input_stream[index + n]
%         write_out(matching_result, match)
% threads_synchronize()
% for index in C:
%     write matching_result to global memory
% \end{lstlisting}

==> tables/change-window.tex <==
\begin{tabular}{@{} l *{5}{r} @{}}
    \toprule
                     &    &
    \multicolumn{2}{r}{\bfseries window size 128}
                     &
    \multicolumn{2}{r@{}}{\bfseries window size 256}                                                                          \\
    \multicolumn{2}{@{}r}{\bfseries Interval}
                     &
    \bfseries CR     &
    \bfseries Change &
    \bfseries CR     &
    \bfseries Change                                                                                                          \\
    \cmidrule(r){1-2}\cmidrule(lr){3-4}\cmidrule(l){5-6}
    \multirow{5}{*}{\rotatebox{90}{CESM}}
                     & 1  & 26.083 & \itshape ref. \visbar{0}   & 31.359 & $+$20.228\% \visbarPos[RedOrange]{20.2}            \\
                     & 2  & 22.987 & $-$11.870\% \visbar{-11.8} & 28.582 & $+$$\phantom{0}$9.581\% \visbarPos[RedOrange]{9.5} \\
                     & 4  & 18.679 & $-$28.387\% \visbar{-28.3} & 22.713 & $-$12.920\% \visbarPos{-12.9}                      \\
                     & 8  & 14.124 & $-$45.848\% \visbar{-45.8} & 16.757 & $-$35.756\% \visbarPos{-35.7}                      \\
                     & 16 & 9.997  & $-$61.672\% \visbar{-61.6} & 11.569 & $-$55.646\% \visbarPos{-55.6}                      \\
    \cmidrule(r){1-2}\cmidrule(lr){3-4}\cmidrule(l){5-6}
    \multirow{5}{*}{\rotatebox{90}{Hurricane}}
                     & 1  & 19.259 & \itshape ref. \visbar{0}   & 22.246 & $+$15.511\% \visbarPos[RedOrange]{15.5}            \\
                     & 2  & 16.890 & $-$12.299\% \visbar{-12.2} & 20.002 & $+$$\phantom{0}$3.857\% \visbarPos[RedOrange]{3.8} \\
                     & 4  & 14.235 & $-$26.087\% \visbar{-26.0} & 16.549 & $-$14.075\% \visbarPos{-14.0}                      \\
                     & 8  & 11.444 & $-$40.577\% \visbar{-40.5} & 13.101 & $-$31.974\% \visbarPos{-31.9}                      \\
                     & 16 & 8.504  & $-$55.842\% \visbar{-55.8} & 9.501  & $-$50.668\% \visbarPos{-50.6}                      \\
    \cmidrule(r){1-2}\cmidrule(lr){3-4}\cmidrule(l){5-6}
    \multirow{5}{*}{\rotatebox{90}{HACC}}
                     & 1  & 10.940 & \itshape ref. \visbar{0}   & 12.527 & $+$14.508\% \visbarPos[RedOrange]{14.5}            \\
                     & 2  & 9.840  & $-$10.061\% \visbar{-10.0} & 11.540 & $+$$\phantom{0}$5.486\% \visbarPos[RedOrange]{5.4} \\
                     & 4  & 7.843  & $-$28.311\% \visbar{-28.3} & 9.004  & $-$17.697\% \visbarPos{-17.6}                      \\
                     & 8  & 6.135  & $-$43.924\% \visbar{-43.9} & 6.895  & $-$36.978\% \visbarPos{-36.9}                      \\
                     & 16 & 4.640  & $-$57.592\% \visbar{-57.5} & 5.093  & $-$53.446\% \visbarPos{-53.4}                      \\
    \cmidrule(r){1-2}\cmidrule(lr){3-4}\cmidrule(l){5-6}
    \multirow{5}{*}{\rotatebox{90}{Nyx}}
                     & 1  & 39.284 & \itshape ref. \visbar{0}   & 49.320 & $+$25.546\% \visbarPos[RedOrange]{25.5}            \\
                     & 2  & 32.766 & $-$16.592\% \visbar{-16.5} & 42.595 & $+$$\phantom{0}$8.428\% \visbarPos[RedOrange]{8.4} \\
                     & 4  & 28.209 & $-$28.192\% \visbar{-28.1} & 35.662 & $-$$\phantom{0}$9.220\% \visbarPos{-9.2}           \\
                     & 8  & 22.730 & $-$42.140\% \visbar{-42.1} & 28.085 & $-$28.508\% \visbarPos{-28.5}                      \\
                     & 16 & 16.902 & $-$56.975\% \visbar{-56.9} & 20.233 & $-$48.496\% \visbarPos{-48.4}                      \\
    \cmidrule(r){1-2}\cmidrule(lr){3-4}\cmidrule(l){5-6}
    \multirow{5}{*}{\rotatebox{90}{QMCPACK}}
                     & 1  & 10.382 & \itshape ref. \visbar{0}   & 12.224 & $+$17.749\% \visbarPos[RedOrange]{17.7}            \\
                     & 2  & 9.169  & $-$11.684\% \visbar{-11.6} & 10.981 & $+$$\phantom{0}$5.777\% \visbarPos[RedOrange]{5.7} \\
                     & 4  & 7.618  & $-$26.617\% \visbar{-26.6} & 8.955  & $-$13.743\% \visbarPos{-13.7}                      \\
                     & 8  & 6.079  & $-$41.449\% \visbar{-41.4} & 7.032  & $-$32.266\% \visbarPos{-32.2}                      \\
                     & 16 & 4.721  & $-$54.527\% \visbar{-54.5} & 5.293  & $-$49.019\% \visbarPos{-49.0}                      \\
    \cmidrule(r){1-2}\cmidrule(lr){3-4}\cmidrule(l){5-6}
    \multirow{5}{*}{\rotatebox{90}{RTM}}
                     & 1  & 20.888 & \itshape ref. \visbar{0}   & 23.914 & $+$14.487\% \visbarPos[RedOrange]{14.5}            \\
                     & 2  & 17.669 & $-$15.409\% \visbar{-15.4} & 20.782 & $-$$\phantom{0}$0.510\% \visbarPos{-0.5}           \\
                     & 4  & 15.422 & $-$26.167\% \visbar{-26.2} & 17.871 & $-$14.443\% \visbarPos{-14.4}                      \\
                     & 8  & 12.907 & $-$38.209\% \visbar{-38.2} & 14.721 & $-$29.525\% \visbarPos{-29.5}                      \\
                     & 16 & 10.609 & $-$49.208\% \visbar{-49.2} & 11.810 & $-$43.459\% \visbarPos{-43.5}                      \\
    \bottomrule
\end{tabular}

==> tables/cmp-compressor-cr.tex <==
\begin{tabular}{@{} lrrrrrr @{}}
        \toprule
        \bfseries Dataset & \bfseries RLE & \bfseries NVCOMP & \bfseries NVCOMP   & \bfseries \thiswork & \bfseries FastLZ
        \\
                          &               & \bfseries LZ4    & \bfseries GDeflate &                     & \bfseries (CPU)
        \\
        \midrule
        CESM
                          &
        1.00              & 14.79         & 20.69            & 28.58              & 27.82                                  \\
        Hurricane         &
        1.01              & 12.03         & 17.13            & 20.00              & 21.52                                  \\
        HACC              &
        1.03              & 6.41          & 9.43             & 11.54              & 11.10                                  \\
        Nyx               &
        1.00              & 31.76         & 40.47            & 42.60              & 54.90                                  \\
        QMCPACK           &
        1.03              & 7.79          & 11.18            & 10.98              & 14.44                                  \\
        RTM               &
        1.01              & 14.46         & 10.47            & 20.78              & 28.73                                  \\
        \bottomrule
\end{tabular}

==> tables/cmp-compressor-time.tex <==
\begin{tabular}{@{} lrrrrrr @{}}
    \toprule
    \bfseries Dataset & \bfseries RLE             & \bfseries NVCOMP & \bfseries NVCOMP   & \bfseries \thiswork & \bfseries FastLZ
    \\
                      &                           & \bfseries LZ4    & \bfseries GDeflate &                     & (CPU)
    \\
    \midrule
    CESM
                      & \multicolumn{1}{c}{73.6}  & 3.01             & 2.87               & 2.77                & 0.45             \\
    Hurricane
                      & \multicolumn{1}{c}{151.8} & 5.97             & 6.60               & 3.22                & 0.42             \\
    HACC
                      & \multicolumn{1}{c}{241.1} & 21.65            & 13.61              & 5.34                & 0.33             \\
    Nyx
                      & \multicolumn{1}{c}{228.3} & 24.18            & 28.47              & 5.39                & 0.51             \\
    QMCPACK
                      & \multicolumn{1}{c}{233.5} & 14.80            & 10.18              & 5.34                & 0.37             \\
    RTM
                      & \multicolumn{1}{c}{191.7} & 6.05             & 6.57               & 3.84                & 0.45             \\
    \bottomrule
\end{tabular}

==> tables/compression_ratio.tex <==
\begin{table}[h]
    \caption{Performance comparison between \textsf{TDC} and existing SOTA compression methods. MD denotes matrix decomposition. DN-1/-2 denote DenseNet-121/-201. Most existing tensor decomposition works do not report results for ResNet-50, VGG-16 and DenseNet on ImageNet.}
    \resizebox{.35\textwidth}{!}{
        \centering
        \footnotesize
        \begin{tabular}{cl|c|c|c}
            \toprule
            \multicolumn{2}{c|}{\multirow{2}{*}{\makecell{\textbf{Model}}}}
                              & \multirow{2}{*}{\makecell{\textbf{Compression}                                            \\
            \textbf{Method}}} & \multirow{2}{*}{\makecell{\textbf{Top-1/Drop}                                             \\
            \textbf{(\%)}}}   & \multirow{2}{*}{\makecell{\textbf{FLOPs}$\downarrow$}}                                    \\
                              &                                                          &           &                    \\
            \midrule
            \multicolumn{1}{c}{\multirow{10}{*}{\rotatebox{90}{ResNet-18}} }
                              & \multicolumn{1}{|c|}{Original \cite{he2016deep}}         & No compr. & 69.75/-0.00 & N/A  \\
                              & \multicolumn{1}{|c|}{FPGM \cite{he2019filter}}           & Pruning   & 68.41/-1.34 & 42\% \\
                              & \multicolumn{1}{|c|}{DSA \cite{ning2020dsa}}             & Pruning   & 68.61/-1.14 & 40\% \\
                              & \multicolumn{1}{|c|}{SCOP \cite{tang2020scop}}           & Pruning   & 68.62/-1.13 & 45\% \\
                              & \multicolumn{1}{|c|}{TRP \cite{xu2020trp}}               & MD        & 65.51/-4.24 & 60\% \\
            % Stable \cite{phan2020stable} & Tucker-CP & 69.07 & 67\%\\
                              & \multicolumn{1}{|c|}{Stable \cite{phan2020stable}}       & CPD       & 69.06/-0.69 & 65\% \\
                              & \multicolumn{1}{|c|}{Opt. TT \cite{yinadmm2021}}         & TTD       & 69.29/-0.46 & 60\% \\
                              & \multicolumn{1}{|c|}{Std. TKD \cite{kim2015compression}} & TKD       & 66.65/-3.10 & 60\% \\
                              & \multicolumn{1}{|c|}{MUSCO \cite{gusak2019automated}}    & TKD       & 69.28/-0.47 & 58\% \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 69.70/-0.05 & 63\% \\
            \midrule
            \multirow{6}{*}{\rotatebox{90}{ResNet-50}}
                              & \multicolumn{1}{|c|}{Original \cite{he2016deep}}         & No compr. & 76.13/-0.00 & N/A  \\
                              & \multicolumn{1}{|c|}{FPGM \cite{he2019filter}}           & Pruning   & 75.59/-0.54 & 42\% \\
                              & \multicolumn{1}{|c|}{HRank \cite{lin2020hrank}}          & Pruning   & 74.98/-1.15 & 44\% \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 77.46/+1.33 & 40\% \\
                              & \multicolumn{1}{|c|}{Stable \cite{phan2020stable}}       & CPD       & 74.66/-1.47 & 60\% \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 76.42/+0.29 & 60\% \\
            \midrule
            \multirow{3}{*}{\rotatebox{90}{VGG-16}}
                              & \multicolumn{1}{|c|}{Original \cite{he2016deep}}         & No compr. & 71.59/-0.00 & N/A  \\
                              & \multicolumn{1}{|c|}{CC \cite{li2021towards} }           & MD        & 68.81/-2.78 & 50\% \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 71.62/+0.03 & 80\% \\\midrule
            \multirow{2}{*}{\rotatebox{90}{DN-1}}
                              & \multicolumn{1}{|c|}{Original \cite{he2016deep}}         & No compr. & 74.43/-0.00 & N/A  \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 76.33/+1.90 & 10\% \\\midrule
            \multirow{2}{*}{\rotatebox{90}{DN-2}}
                              & \multicolumn{1}{|c|}{Original \cite{he2016deep}}         & No compr. & 76.88/-0.00 & N/A  \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 76.92/+0.04 & 10\% \\\bottomrule
        \end{tabular}
    }
    \label{tab:accuracy}
\end{table}

==> tables/compression_time.tex <==
\begin{table}[h]
    \caption{Performance comparison between \textsf{TDC} and existing SOTA compression methods. MD denotes matrix decomposition. DN-1/-2 denote DenseNet-121/-201. Most existing tensor decomposition works do not report results for ResNet-50, VGG-16 and DenseNet on ImageNet.}
    \resizebox{.35\textwidth}{!}{
        \centering
        \footnotesize
        \begin{tabular}{cl|c|c|c}
            \toprule
            \multicolumn{2}{c|}{\multirow{2}{*}{\makecell{\textbf{Model}}}}
                              & \multirow{2}{*}{\makecell{\textbf{Compression}                                            \\
            \textbf{Method}}} & \multirow{2}{*}{\makecell{\textbf{Top-1/Drop}                                             \\
            \textbf{(\%)}}}   & \multirow{2}{*}{\makecell{\textbf{FLOPs}$\downarrow$}}                                    \\
                              &                                                          &           &                    \\
            \midrule
            \multicolumn{1}{c}{\multirow{10}{*}{\rotatebox{90}{ResNet-18}} }
                              & \multicolumn{1}{|c|}{Original \cite{he2016deep}}         & No compr. & 69.75/-0.00 & N/A  \\
                              & \multicolumn{1}{|c|}{FPGM \cite{he2019filter}}           & Pruning   & 68.41/-1.34 & 42\% \\
                              & \multicolumn{1}{|c|}{DSA \cite{ning2020dsa}}             & Pruning   & 68.61/-1.14 & 40\% \\
                              & \multicolumn{1}{|c|}{SCOP \cite{tang2020scop}}           & Pruning   & 68.62/-1.13 & 45\% \\
                              & \multicolumn{1}{|c|}{TRP \cite{xu2020trp}}               & MD        & 65.51/-4.24 & 60\% \\
            % Stable \cite{phan2020stable} & Tucker-CP & 69.07 & 67\%\\
                              & \multicolumn{1}{|c|}{Stable \cite{phan2020stable}}       & CPD       & 69.06/-0.69 & 65\% \\
                              & \multicolumn{1}{|c|}{Opt. TT \cite{yinadmm2021}}         & TTD       & 69.29/-0.46 & 60\% \\
                              & \multicolumn{1}{|c|}{Std. TKD \cite{kim2015compression}} & TKD       & 66.65/-3.10 & 60\% \\
                              & \multicolumn{1}{|c|}{MUSCO \cite{gusak2019automated}}    & TKD       & 69.28/-0.47 & 58\% \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 69.70/-0.05 & 63\% \\
            \midrule
            \multirow{6}{*}{\rotatebox{90}{ResNet-50}}
                              & \multicolumn{1}{|c|}{Original \cite{he2016deep}}         & No compr. & 76.13/-0.00 & N/A  \\
                              & \multicolumn{1}{|c|}{FPGM \cite{he2019filter}}           & Pruning   & 75.59/-0.54 & 42\% \\
                              & \multicolumn{1}{|c|}{HRank \cite{lin2020hrank}}          & Pruning   & 74.98/-1.15 & 44\% \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 77.46/+1.33 & 40\% \\
                              & \multicolumn{1}{|c|}{Stable \cite{phan2020stable}}       & CPD       & 74.66/-1.47 & 60\% \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 76.42/+0.29 & 60\% \\
            \midrule
            \multirow{3}{*}{\rotatebox{90}{VGG-16}}
                              & \multicolumn{1}{|c|}{Original \cite{he2016deep}}         & No compr. & 71.59/-0.00 & N/A  \\
                              & \multicolumn{1}{|c|}{CC \cite{li2021towards} }           & MD        & 68.81/-2.78 & 50\% \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 71.62/+0.03 & 80\% \\\midrule
            \multirow{2}{*}{\rotatebox{90}{DN-1}}
                              & \multicolumn{1}{|c|}{Original \cite{he2016deep}}         & No compr. & 74.43/-0.00 & N/A  \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 76.33/+1.90 & 10\% \\\midrule
            \multirow{2}{*}{\rotatebox{90}{DN-2}}
                              & \multicolumn{1}{|c|}{Original \cite{he2016deep}}         & No compr. & 76.88/-0.00 & N/A  \\
                              & \multicolumn{1}{|c|}{TDC}                                & TKD       & 76.92/+0.04 & 10\% \\\bottomrule
        \end{tabular}
    }
    \label{tab:accuracy}
\end{table}

==> tables/dataset.tex <==
\begin{tabular}{@{} >{\bfseries\scshape}lrr @{}}
    % \toprule
                                        & \bfseries datum size               & \bfseries \#fields                        \\[-.4ex]
    \TABLETITLE datasets                &
    \TABLETITLE dimensions              &
    \TABLETITLE examples(s)                                                                                              \\%[1ex]
    \midrule
    \TABLECAPTION cosmology             & \TABLECAPTION 1,071.75 MB          & \TABLECAPTION 6 in total                  \\[-.6ex]
    HACC                                & 280,953,867                        & xx, vx                                    \\
    \TABLECAPTION cosmology             & \TABLECAPTION 512 MB               & \TABLECAPTION 6 in total                  \\[-.6ex]
    Nyx                                 & 512$\times$512$\times$512          & baryon\_density                           \\
    \TABLECAPTION climate               & \TABLECAPTION 381.47 MB            & \TABLECAPTION 13 in total                 \\[-.6ex]
    Hurricane                           & 4$\times$100$\times$500$\times$500 & CLDICE, QRAIN                             \\
    \TABLECAPTION petroleum exploration & \TABLECAPTION 180.73 MB            & \TABLECAPTION 3 in total (3600 snapshots) \\[-.6ex]
    RTM                                 & 449$\times$449$\times$235          & snapshot\_0600-1000                       \\
    \bottomrule
\end{tabular}

==> tables/evolving.tex <==
\begin{tabular}{ @{} l @{} r *{5}{r} @{} }
    \toprule
     & \rotatebox{90}{\bfseries Optim.}
     & \rottitle{Match}{Time}
     & \rottitle{Enc.}{Time}
     & \rottitle{D2H}{Time}
     & \rottitle{Overall}{Time}
     & \rottitle{Speed}{-up}
    \\
    \midrule
    \multirow{5}{*}{\rotatebox{90}{CESM}}
     & \multicolumn{1}{r}{wsize128}     & 13.821  & 6.010   & 1.392  & 21.223
     & \SpeedupBar{1.00}                                                          \\
     & \multicolumn{1}{r}{wsize256}     & 14.595  & 7.704   & 1.152  & 23.451
     & \SpeedupBar{0.91}                                                          \\
     & \multicolumn{1}{r}{shmem}        & 7.892   & 5.000   & 0.990  & 13.882
     & \SpeedupBar{1.53}                                                          \\
     & \multicolumn{1}{r}{enc-kernel}   & 14.645  & 0.418   & -      & 15.063
     & \SpeedupBar{1.41}                                                          \\
     & \multicolumn{1}{r}{final}        & 8.966   & 0.398   & -      & 9.364
     & \SpeedupBar{2.27}                                                          \\
    \midrule
    \multirow{5}{*}{\rotatebox{90}{Hurrica}}
     & \multicolumn{1}{r}{wsize128}     & 50.928  & 28.049  & 4.872  & 83.849   &
    \SpeedupBar{1.00}                                                             \\
     & \multicolumn{1}{r}{wsize256}     & 53.365  & 31.738  & 4.840  & 89.944   &
    \SpeedupBar{0.93}                                                             \\
     & \multicolumn{1}{r}{shmem}        & 28.494  & 23.068  & 3.257  & 54.820   &
    \SpeedupBar{1.53}                                                             \\
     & \multicolumn{1}{r}{enc-kernel}   & 45.371  & 0.556   & -      & 45.927   &
    \SpeedupBar{1.83}                                                             \\
     & \multicolumn{1}{r}{final}        & 30.492  & 0.575   & -      & 31.067   &
    \SpeedupBar{2.70}                                                             \\
    \midrule
    \multirow{5}{*}{\rotatebox{90}{HACC}}
     & \multicolumn{1}{r}{wsize128}     & 627.484 & 451.519 & 53.758 & 1132.761 &
    \SpeedupBar{1.00}                                                             \\
     & \multicolumn{1}{r}{wsize256}     & 656.485 & 489.577 & 46.334 & 1192.396 &
    \SpeedupBar{0.95}                                                             \\
     & \multicolumn{1}{r}{shmem}        & 234.463 & 377.588 & 31.603 & 643.653  &
    \SpeedupBar{1.76}                                                             \\
     & \multicolumn{1}{r}{enc-kernel}   & 370.517 & 3.617   & -      & 374.134  &
    \SpeedupBar{3.03}                                                             \\
     & \multicolumn{1}{r}{final}        & 206.857 & 3.449   & -      & 210.306  &
    \SpeedupBar{5.39}                                                             \\
    \midrule
    \multirow{5}{*}{\rotatebox{90}{Nyx}}
     & \multicolumn{1}{r}{wsize128}     & 260.234 & 114.774 & 27.784 & 402.792  &
    \SpeedupBar{1.00}                                                             \\
     & \multicolumn{1}{r}{wsize256}     & 277.750 & 139.822 & 22.831 & 440.403  &
    \SpeedupBar{0.91}                                                             \\
     & \multicolumn{1}{r}{shmem}        & 108.239 & 130.144 & 16.907 & 255.291  &
    \SpeedupBar{1.58}                                                             \\
     & \multicolumn{1}{r}{enc-kernel}   & 157.728 & 0.517   & -      & 158.245  &
    \SpeedupBar{2.55}                                                             \\
     & \multicolumn{1}{r}{final}        & 99.082  & 0.531   & -      & 99.613   &
    \SpeedupBar{4.04}                                                             \\
    \midrule
    \multirow{5}{*}{\rotatebox{90}{QMCPACK}}
     & \multicolumn{1}{r}{wsize128}     & 344.090 & 265.021 & 39.138 & 648.248  &
    \SpeedupBar{1.00}                                                             \\
     & \multicolumn{1}{r}{wsize256}     & 350.050 & 294.561 & 37.941 & 682.552  &
    \SpeedupBar{0.95}                                                             \\
     & \multicolumn{1}{r}{shmem}        & 155.450 & 273.169 & 20.151 & 448.769  &
    \SpeedupBar{1.44}                                                             \\
     & \multicolumn{1}{r}{enc-kernel}   & 202.702 & 2.265   & -      & 204.967  &
    \SpeedupBar{3.16}                                                             \\
     & \multicolumn{1}{r}{final}        & 116.042 & 2.164   & -      & 118.206  &
    \SpeedupBar{5.48}                                                             \\
    \midrule
    \multirow{5}{*}{\rotatebox{90}{RTM}}
     & \multicolumn{1}{r}{wsize128}     & 93.894  & 91.822  & 8.865  & 194.581  &
    \SpeedupBar{1.00}                                                             \\
     & \multicolumn{1}{r}{wsize256}     & 93.538  & 84.808  & 9.372  & 187.718  &
    \SpeedupBar{1.04}                                                             \\
     & \multicolumn{1}{r}{shmem}        & 57.595  & 81.134  & 6.354  & 145.083  &
    \SpeedupBar{1.34}                                                             \\
     & \multicolumn{1}{r}{enc-kernel}   & 56.116  & 0.676   & -      & 56.792   &
    \SpeedupBar{3.43}                                                             \\
     & \multicolumn{1}{r}{final}        & 48.588  & 0.802   & -      & 49.390   &
    \SpeedupBar{3.94}                                                             \\
    \bottomrule
\end{tabular}

==> tables/parameters.tex <==
\begin{table}[!htp]\centering
    \caption{Generated by Spread-LaTeX}\label{tab: }
    \scriptsize
    \begin{tabular}{lrrrrrrrrrrrrrr}\toprule
                          & data chunk size & 2048       &        &             & 4096       &        &             & 8192       &        &             & 16384      &        &             \\\cmidrule{2-3}\cmidrule{6-6}\cmidrule{9-12}
                          & window\_size    & uint8/char & uint16 & uint32/foat & uint8/char & uint16 & uint32/foat & uint8/char & uint16 & uint32/foat & uint8/char & uint16 & uint32/foat \\\cmidrule{2-14}
        hurr-quantization & 32              & 3.14       & 3.77   & 3.58        & 3.18       & 3.84   & 3.66        &            & 3.88   & 3.7         &            &        & 3.72        \\\cmidrule{1-8}\cmidrule{10-14}
                          & 64              & 3.79       & 4.39   & 4.05        & 3.86       & 4.5    & 4.18        &            & 4.56   & 4.25        &            &        & 4.28        \\\cmidrule{2-8}\cmidrule{10-14}
                          & 128             & 4.39       & 4.91   & 4.44        & 4.51       & 5.09   & 4.64        &            & 5.18   & 4.75        &            &        & 4.81        \\\cmidrule{2-8}\cmidrule{10-14}
                          & 255             & 4.89       & 5.32   & 4.78        & 5.07       & 5.59   & 5.15        &            & 5.73   & 5.36        &            &        & 5.47        \\\cmidrule{2-8}\cmidrule{10-14}
        hacc-quantization & 32              & 1.55       & 1.67   & 1.59        & 1.55       & 1.68   & 1.6         &            & 1.68   & 1.61        &            &        & 1.61        \\\cmidrule{1-8}\cmidrule{10-14}
                          & 64              & 1.71       & 1.82   & 1.71        & 1.72       & 1.84   & 1.73        &            & 1.85   & 1.74        &            &        & 1.75        \\\cmidrule{2-8}\cmidrule{10-14}
                          & 128             & 1.87       & 1.97   & 1.83        & 1.88       & 2      & 1.86        &            & 2.02   & 1.88        &            &        & 1.89        \\\cmidrule{2-8}\cmidrule{10-14}
                          & 255             & 2.01       & 2.12   & 1.92        & 2.03       & 2.18   & 1.99        &            & 2.2    & 2.03        &            &        & 2.05        \\\cmidrule{2-8}\cmidrule{10-14}
        nyx-quantization  & 32              & 3.97       & 5.07   & 4.8         & 4.04       & 5.2    & 4.95        &            & 5.27   & 5.02        &            &        & 5.06        \\\cmidrule{1-8}\cmidrule{10-14}
                          & 64              & 5.06       & 6.18   & 5.73        & 5.19       & 6.42   & 6           &            & 6.54   & 6.14        &            &        & 6.21        \\\cmidrule{2-8}\cmidrule{10-14}
                          & 128             & 6.14       & 7.19   & 6.52        & 6.36       & 7.57   & 6.99        &            & 7.79   & 7.25        &            &        & 7.38        \\\cmidrule{2-8}\cmidrule{10-14}
                          & 255             & 7.08       & 8.03   & 7.11        & 7.46       & 8.65   & 7.94        &            & 9.01   & 8.42        &            &        & 8.64        \\\cmidrule{2-8}\cmidrule{10-14}
        tpch-integer      & 32              & 1.31       & 1.25   & 1.29        & 1.32       & 1.26   & 1.3         &            & 1.26   & 1.3         &            &        & 1.3         \\\cmidrule{1-8}\cmidrule{10-14}
                          & 64              & 1.37       & 1.3    & 1.34        & 1.38       & 1.31   & 1.35        &            & 1.31   & 1.35        &            &        & 1.36        \\\cmidrule{2-8}\cmidrule{10-14}
                          & 128             & 1.43       & 1.34   & 1.38        & 1.44       & 1.35   & 1.39        &            & 1.36   & 1.4         &            &        & 1.41        \\\cmidrule{2-8}\cmidrule{10-14}
                          & 255             & 1.5        & 1.38   & 1.41        & 1.51       & 1.39   & 1.43        &            & 1.4    & 1.44        &            &        & 1.45        \\\cmidrule{2-8}\cmidrule{10-14}
        tpch-string       & 32              & 1.55       & 1.58   & 1.46        & 1.56       & 1.59   & 1.47        &            & 1.6    & 1.48        &            &        & 1.48        \\\cmidrule{1-8}\cmidrule{10-14}
                          & 64              & 2.02       & 1.96   & 1.72        & 2.04       & 1.99   & 1.76        &            & 2.01   & 1.78        &            &        & 1.79        \\\cmidrule{2-8}\cmidrule{10-14}
                          & 128             & 2.57       & 2.43   & 2.03        & 2.62       & 2.5    & 2.12        &            & 2.54   & 2.17        &            &        & 2.2         \\\cmidrule{2-8}\cmidrule{10-14}
                          & 255             & 3.08       & 2.84   & 2.27        & 3.19       & 3      & 2.47        &            & 3.09   & 2.58        &            &        & 2.64        \\\cmidrule{2-8}\cmidrule{10-14}
        rtm               & 32              &            &        &             &            &        &             &            &        &             &            &        &             \\\cmidrule{1-2}
                          & 64              &            &        &             &            &        &             &            &        &             &            &        &             \\
                          & 128             &            &        &             &            &        &             &            &        &             &            &        &             \\
                          & 255             &            &        &             &            &        &             &            &        &             &            &        &             \\\midrule
        \bottomrule
    \end{tabular}
\end{table}

==> tables_batch2/tp.tex <==
\begin{tabular}{ @{} lr *{3}{r}  *{3}{r} *{3}{r} *{3}{r}@{}}\toprule
                                         &
                                         &
    \multicolumn{3}{c}{chunk size: 2048} &
    \multicolumn{3}{c}{chunk size: 4096} &
    \multicolumn{3}{c}{chunk size: 8192} &
    \multicolumn{3}{c@{}}{chunk size: 16384}                                                                                                                                                           \\
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(l){12-14}
    \multicolumn{2}{@{}r}{window size $\downarrow$}
                                         & 1 byte & 2 bytes   & 4 bytes     & 1 byte      & 2 bytes   & 4 bytes    & 1 byte      & 2 bytes & 4 bytes    & 1 byte      & 2 bytes & 4 bytes              \\\midrule
    hurr                                 & 32     & 8.13/4.87 & 14.85/9.57  & 29/18.07    & 6.87/3.1  & 14.82/8.38 & 27.98/17.44 & n/a     & 11.26/4.37 & 26.62/13.29 & n/a     & n/a     & 15.99/7.55 \\
    quant                                & 64     & 4.63/2.93 & 8.9/5.55    & 17.53/11.18 & 4.47/2.19 & 8.64/5.28  & 17.15/10.95 & n/a     & 7.4/3.11   & 16.64/9.22  & n/a     & n/a     & 11.84/5.62 \\
                                         & 128    & 2.52/1.6  & 4.87/3.08   & 11.04/6.73  & 2.43/1.33 & 4.72/2.94  & 10.08/6.31  & n/a     & 4.3/1.95   & 9.45/5.68   & n/a     & n/a     & 7.4/3.71   \\
                                         & 255    & 1.39/0.87 & 2.76/1.75   & 6.95/4.37   & 1.33/0.79 & 2.6/1.6    & 5.7/3.63    & n/a     & 2.34/1.13  & 5.3/3.26    & n/a     & n/a     & 4.33/2.25  \\
    \cmidrule(l){2-14}
    hacc                                 & 32     & 7.35/4.16 & 13.81/8.49  & 28.96/18.14 & 5.83/2.63 & 13.13/7.54 & 27.48/15.49 & n/a     & 9.31/3.42  & 24.57/10.58 & n/a     & n/a     & 14.5/6.06  \\
    quant                                & 64     & 4.47/2.75 & 8.21/5.31   & 19.19/11.44 & 4.1/2.08  & 8.15/5.1   & 19.07/11.42 & n/a     & 6.57/2.74  & 17.36/8.39  & n/a     & n/a     & 11.12/5.27 \\
                                         & 128    & 2.56/1.69 & 4.76/3.05   & 12.36/6.31  & 2.59/1.37 & 4.65/3.04  & 11.06/6.74  & n/a     & 4.21/1.98  & 11.12/6.03  & n/a     & n/a     & 7.87/3.58  \\
                                         & 255    & 1.5/0.95  & 2.68/1.83   & 7.4/4.37    & 1.5/0.82  & 2.68/1.67  & 6.65/3.93   & n/a     & 2.49/1.21  & 6/3.51      & n/a     & n/a     & 4.93/2.45  \\
    \cmidrule(l){2-14}
    nyn/a                                & 32     & 9.53/6.04 & 15.65/10.14 & 30.08/19.05 & 7.53/3.95 & 15.75/9.05 & 30.26/18.76 & n/a     & 12.44/5.62 & 29.18/14.67 & n/a     & n/a     & 18.13/8.36 \\
    quant                                & 64     & 5.69/3.57 & 9.44/6.15   & 19.81/11.6  & 5.4/2.83  & 9.3/6.15   & 18/11.4     & n/a     & 8.12/3.75  & 17.94/10.79 & n/a     & n/a     & 12.9/6.33  \\
                                         & 128    & 3.05/1.92 & 5.48/3.57   & 11.29/7.1   & 3.08/1.66 & 5.91/3.38  & 10.31/6.77  & n/a     & 5.01/2.47  & 10.16/6.45  & n/a     & n/a     & 8.71/4.61  \\
                                         & 255    & 1.76/1.03 & 3.56/2.07   & 6.94/4.86   & 1.67/0.91 & 3.17/1.9   & 6.6/4.13    & n/a     & 3.07/1.4   & 6.3/3.87    & n/a     & n/a     & 5.29/2.82  \\
    \cmidrule(l){2-14}
    tpch                                 & 32     & 7.07/3.93 & 12.06/8.3   & 25.42/14.87 & 5.21/2.25 & 11.66/6.21 & 21.4/13.49  & n/a     & 7.67/3.09  & 19.39/9.29  & n/a     & n/a     & 10.45/5.01 \\
    integer                              & 64     & 4.38/2.68 & 7.87/5.11   & 16.32/10.2  & 3.76/1.74 & 7.53/4.52  & 14.58/9.78  & n/a     & 5.89/2.38  & 14.24/7.05  & n/a     & n/a     & 8.23/4.19  \\
                                         & 128    & 2.41/1.57 & 4.75/3.02   & 10.22/6.31  & 2.24/1.14 & 4.46/2.76  & 9.23/5.56   & n/a     & 3.81/1.68  & 8.39/5.01   & n/a     & n/a     & 6.44/3.11  \\
                                         & 255    & 1.32/0.85 & 2.76/1.72   & 6.67/3.97   & 1.24/0.68 & 2.41/1.57  & 5.76/3.45   & n/a     & 2.14/1.02  & 4.99/3.08   & n/a     & n/a     & 3.77/2     \\
    \cmidrule(l){2-14}
    tpch                                 & 32     & 7.08/4.23 & 12.52/7.96  & 22.92/13.82 & 5.32/2.46 & 11.39/6.16 & 21.11/12.62 & n/a     & 7.98/3.51  & 18.95/8.42  & n/a     & n/a     & 9.96/4.83  \\
    string                               & 64     & 4.71/3.06 & 8.35/5.21   & 15.15/9.5   & 4.16/1.97 & 7.58/5.09  & 15.56/9.23  & n/a     & 6.29/2.88  & 13.98/6.83  & n/a     & n/a     & 8.22/4.13  \\
                                         & 128    & 2.4/1.74  & 4.77/3.28   & 10.71/5.97  & 2.57/1.31 & 4.71/3.13  & 9.43/5.68   & n/a     & 3.98/1.98  & 8.15/4.84   & n/a     & n/a     & 5.74/3.5   \\
                                         & 255    & 1.41/0.94 & 2.58/1.83   & 6.91/3.74   & 1.42/0.79 & 2.62/1.72  & 6.06/3.31   & n/a     & 2.31/1.19  & 4.74/3.33   & n/a     & n/a     & 3.68/2.26  \\
    \cmidrule(l){2-14}
    rtm                                  & 32     & 7.31/4.23 & 14.27/9     & 28.35/17.63 & 6.05/2.79 & 13.92/7.54 & 28.57/17.17 & n/a     & 11.22/3.91 & 26.63/13.14 & n/a     & n/a     & 16.23/7.44 \\
    float32                              & 64     & 4.48/2.85 & 9.27/5.52   & 17.69/11.15 & 3.92/2.18 & 8.3/5.1    & 17.4/10.9   & n/a     & 7.02/3.04  & 16.77/9.08  & n/a     & n/a     & 12.37/5.52 \\
                                         & 128    & 2.46/1.77 & 4.89/3.38   & 10.81/6.84  & 2.37/1.39 & 4.71/3.07  & 9.99/6.35   & n/a     & 4.17/1.89  & 9.59/5.61   & n/a     & n/a     & 7.52/3.65  \\
                                         & 255    & 1.35/0.98 & 3.07/2.03   & 8.05/4.82   & 1.31/0.82 & 3.06/1.8   & 6.08/3.82   & n/a     & 2.55/1.28  & 5.78/3.28   & n/a     & n/a     & 4.47/2.57  \\
    \bottomrule
\end{tabular}

